Learning to Better Segment Objects from Unseen Classes with Unlabeled Videos

The ability to localize and segment objects from unseen classes would open the door to new applications, such as autonomous object learning in active vision. Nonetheless, improving the performance on unseen classes requires additional training data, while manually annotating the objects of the unseen classes can be labor-extensive and expensive. In this paper, we explore the use of unlabeled video sequences to automatically generate training data for objects of unseen classes. It is in principle possible to apply existing video segmentation methods to unlabeled videos and automatically obtain object masks, which can then be used as a training set even for classes with no manual labels available. However, our experiments show that these methods do not perform well enough for this purpose. We therefore introduce a Bayesian method that is specifically designed to automatically create such a training set: Our method starts from a set of object proposals and relies on (non-realistic) analysis-by-synthesis to select the correct ones by performing an efficient optimization over all the frames simultaneously. Through extensive experiments, we show that our method can generate a high-quality training set which significantly boosts the performance of segmenting objects of unseen classes. We thus believe that our method could open the door for open-world instance segmentation using abundant Internet videos.

==> 2.Related_work.tex <==

In this section, we first review recent works on instance segmentation from color images, especially those targeting new classes. We also review self-learning methods on unlabeled images. Finally, we review several works for video object segmentation as this topic is closely related to our approach.


\paragraph{Image-level Instance Segmentation.}

While state-of-the-art methods for object detection and segmentation~\cite{he2017mask, tian2020conditional, wang2020solo} rely on large amounts of manually labeled images, a few works aim at reducing the annotation burden for learning to detect and segment object classes.  They however still require manual annotations: Weakly-supervised methods require no mask annotations but bounding boxes annotations~\cite{hu2018learning, Kuo2019ShapeMaskLT, Zhou2020LearningSP} and few-shot methods require a (small) number of manual object masks~\cite{Fan2020FGNFG,Yan2019MetaRT}.


\paragraph{Self-Learning on Unlabeled Data.}


Recently, several methods have been proposed to explore self-supervision using unlabeled static images. They use data distillation~\cite{Radosavovic2018DataDT}, unlabeled images from the web~\cite{li2020improving}, consistency across image flipping~\cite{jeong2019consistency}, or an estimate of the uncertainty of prediction~\cite{neverova2019correlated}. While such approaches are very interesting, unlabelled videos are easily available and have the potential to make the results much more reliable. We compare our method against the most representative methods in our experiments and show we achieve much better performance.



Another type of approach proceeds in a bottom-up fashion by grouping pixels with similar colors or image features to generate masks~\cite{burgess2019monet,greff2019multi,slot_attention,pham2018bayesian,wong2020identifying}. However, this can be easily affected by local textures or colors, and some of these methods have been demonstrated on synthetic images only. Because it starts from a pre-trained instance segmentation model, our approach is much more robust.



Like us, some methods leverage unlabeled videos for on urban scene segmentation~\cite{Chen2020LeveragingSL} and face and human detection\cite{jin2018unsupervised}. However, these works only focus on how to enhance the model performance on the existing classes and do not consider novel classes.  \cite{ovsep2019large} makes use of stereo video data together with depth information to reconstruct a static background, then object proposals are generated from the foreground regions by subtraction.  While this is an interesting approach, they require depth data and static backgrounds.




\paragraph{Video Object Segmentation.}

Our  work  also  relates  to   One-Shot,  Zero-Shot  video  object
segmentation~(VOS) and saliency-based video object segmentation. One-Shot VOS aims at segmenting the objects in the video when the ground truth segmentation is given for a frame. One-Shot VOS methods typically warp the provided segmentation to other frames~\cite{caelles2017one, uvc_2019, wang2019learning}. They thus require manual  annotations and cannot generate new predictions if new objects appear. Some Zero-Shot methods~\cite{cheng2017segflow, oh2019video, ventura2019rvos, voigtlaender2019feelvos} are trained with video labels on seen classes and are able to generalize to unseen classes, but video labeling is very labor-extensive. Some methods look for salient regions in videos~\cite{Chen_TransferSeg_2018, croitoru2017unsupervised, dave2019towards, faktor2014video, jain2017fusionseg, Koh2017Primary, lu2020learning, papazoglou2013fast}, as salient regions tend to correspond to objects. However, saliency prediction has two major limitations for our purpose: (a) It can be fooled by non-salient camouflaged objects. (b) Two adjacent objects would be merged into a single salient region, while we want to identify them individually.

Like us, a few methods already adopt a proposal-based approach~\cite{bergmann2019tracking, luiten2020unovost, milan2015joint}, but rely on classical tracking algorithms to track the proposals such as tracklets. By contrast, our approach relies on analysis-by-synthesis. Analysis-by-synthesis is an old concept in computer vision, but has been recently increasingly popular. By aiming at explaining the whole image, it can exploit more information. Moreover, it is conceptually simple and requires few easy-to-fix hyper-parameters. We show in our experiments that our method performs better than the state-of-the-art video object segmentation method UnOVOST~\cite{luiten2020unovost} for the purpose of generating object masks.




